Top-quark electroweak interactions at high energy

Modified interactions in the electroweak sector may lead to scattering amplitudes that grow with energy compared to their Standard Model (SM) counterparts. We present a detailed study of all $2\to2$ scattering amplitudes involving at least one top quark and a pair of EW bosons. We analyse the high energy behaviour of the amplitudes using the Standard Model Effective Field Theory (SMEFT) to parametrise the departures from the SM. We discuss the origin of the energy growth that arise from effective contact interactions by appealing to the Goldstone equivalence theorem and find that the amplitudes obey expected patterns of (non-)interference. The results are connected to unitary-violating behaviour in the framework of anomalous SM interactions. Therein, we identify the appearance of additional growth due to the violation of $SU(2)$ gauge symmetry that leads to substantial differences between the SMEFT and the anomalous couplings approaches. We also discuss the embeddings of the scattering amplitudes into physical collider processes, presenting the parametric SMEFT sensitivity to relevant top quark operators and paying special attention to the extent to which the high energy behaviour of the $2\to2$ amplitude is retained in the actual processes accessible at colliders. The effective $W$ approximation is exploited to gain analytical insight into the embeddings of the $2\to2$ helicity amplitudes. Finally, we provide a compendium of processes detailing numerous directions in which the SMEFT parameter space can be accessed through high energy top quark processes in current and future colliders.

==> EW_subprocesses.tex <==
\subsection{$\mathbf{b \, W \to t \, h}$ scattering
\label{subsec:bwth}}
	\begin{figure}[h!]
		\centering
        \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/bwth_1}
        } 
        \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/bwth_3}
        }
        \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/bwth_2}
        }
 
		\caption{SM diagrams for the $b W \to t h$ subprocess. \label{bwth_sm}}
	\end{figure}
\noindent This process probes the coupling of the top quark with the Higgs and with the $W$, as can be seen in Fig. \ref{bwth_sm}, depicting the contributing unitary gauge Feynman diagrams. The third diagram can be neglected in principle, since the b quark is nearly massless and therefore its coupling to the Higgs negligible. The coupling to the $W$ is present in every diagram, meaning that a modification to the SM coupling cannot lead to non-unitary behaviour, but just provide an overall factor to the amplitude. The helicity amplitude table for this process was provided earlier in Table~\ref{tab:bwth}. From the SMEFT perspective the table can be easily interpreted in terms of contact terms and helicity flips, as previously explained. For example, The leading energy growth proportional to $\sqrt{s(s+t)}$ comes from the $\Opp{\phi Q}{(3)}$ contribution to the  longitudinal, left handed configuration, $(-1,0,-1)$. This is attributed to the dimension-6 contact term involving the Higgs and a charged Goldstone boson induced by this operator,
\begin{equation}
    \label{eq:OphiQ3}
    \Opp{\phi Q}{(3)} = i\big(\phi^\dagger\lra{D}_\mu\,\tau_{\sss I}\phi\big)
     \big(\bar{Q}\,\gamma^\mu\,\tau^{\sss I}Q\big) \quad \to \quad h \, \partial_\mu G_+ \, \bar{t}_L \gamma^\mu b_L \, +\text{h.c.}
\end{equation}
	From the AC perspective, we can modify the $btW$, the $tth$ and the $WWh$ vertices. As already mentioned, the $btW$ coupling just gives an overall factor to the amplitude, while the $tth$ coupling and $WWh$ in the SM are related such that there is a cancellation of energy growth. Specifically, there is a contribution to the helicity configuration $(-1,0,1)$, 
	\begin{equation}
		\sqrt{-t}\,(2m_W^2 y_t - g_{Wh} m_t),
	\end{equation}
which cancels when assigning the SM values to the couplings. There is no higher degree energy growth due to ACs for this process.

	Mapping the SMEFT to the ACs, we can see that the Yukawa operator $\Op{t \phi}=(\phi^\dagger\phi-\frac{v^2}{2})\bar{Q}t\tilde{\phi}$, which modifies the $tth$ coupling, indeed gives a contribution proportional to $\sqrt{-t}$ in the same helicity configuration, as discussed in Section~\ref{subsubsec:egrowthandcontact}. This operator modifies both the $tth$ vertex and the mass of the top, but does so with different contributions due to combinatorics (the operator has 3 Higgs doublets, so there is only one way of obtaining a mass term by selecting the vev in each of them, while one can select the dynamical Higgs in 3 different ways). If the alterations were equal, one would have no energy growing behaviour. Our definition of the operator modifies $y_t$, but not $m_W, m_t$ or $k_W$. The exact anomalous coupling that is modified is basis dependent, \textit{i.e.}, trading away the Yukawa operator with a Higgs doublet field redefinition would cause the appearance of new operators that in the end would modify $m_W$ and $k_W$. Alternatively, removing the $-v^2/2$ component leads to a simultaneous modification of $y_t$ and $m_t$. All cases lead to the same physical effect. As mentioned in Section~\ref{subsubsec:egrowthandcontact}, the energy growth can also be understood in terms of a $btG^+h$ contact term in Feynman gauge. 
%
\subsection{$\mathbf{b \, W \to t \, Z}$ scattering
\label{subsec:bwtz}}
	\begin{figure}[h!]
		\centering
		\subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/bwtz_1}
        }  \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/bwtz_2}
        }
        \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/bwtz_3}
        }
		\caption{SM diagrams for the $b W \to t Z$ subprocess. \label{bwtz_sm}}
	\end{figure}
\noindent This process is very similar to the previous one, with a $Z$ boson replacing the Higgs boson, as can be seen in Fig. \ref{bwtz_sm}, with the exception that the third diagram, which couples the b quark to the Z, does play a role. The $btW$ vertex is still present in every diagram and its modification does not lead to energy growth. From the AC perspective, one can modify the $ttZ$, $WWZ$ and $bbZ$ couplings. In general, one can modify the left and right handed $Z$ couplings to the fermions separately. In the SM these interactions are related by Gauge invariance and the Higgs mechanism. In particular, the left handed $b$ and $t$ couplings are connected because of the fact that they form an $SU(2)$ doublet. Modifying these 2 couplings independently constitutes an additional source of EW symmetry breaking beyond the SM and, as a consequence, leads to unitarity violation. The contributions to the offending helicity configurations $(-1,-1,-1,0)$ and $(-1,0,-1,-1)$ are proportional to 
    \begin{equation}
        \sqrt{-t}\,(\gzbl - \gztl + \gwz) \, ,
    \end{equation}
    and to the $(-1,0,1,0)$ helicity amplitude are proportional to
    \begin{equation}
        \sqrt{-t}\,(2m_W^2(\gzbl - \gztr + \gwz) - \gwz m_Z^2) \, .
    \end{equation}
    For this amplitude there is also a $E^2$ effect in the helicity configuration $(-1,0,-1,0)$ proportional to
    \begin{equation}
        \sqrt{s(s+t)}\,(\gzbl - \gztl + \gwz) \, .
    \end{equation}
The simultaneous appearance of $\gzbl,\,\gztr$ and $\gwz$ highlights the fact that both the gauge-fermion and gauge self-interactions arise from the same non-Abelian gauge theory and independent modifications of these two also constitute a violation of gauge invariance. 

Within the Gauge-invariant SMEFT framework, one can verify in Table~\ref{tab:bwtz} that in the pure Gauge scattering, i.e. when both weak bosons are transversely polarised, the only source of energy growth comes from operators that introduce new Lorentz structures, such as the dipole and triple gauge operators. As mentioned in Section~\ref{subsubsec:egrowthandcontact}, if one takes into account these new Lorentz structures in an anomalous coupling framework but omits the relevant contact term $bWtZ$, higher powers of energy growth $\propto E^3$ occur in the fully longitudinal configurations. 
    The scattering of longitudinal weak bosons, can be connected in Feynman gauge to the appearance of contact terms involving the Goldstones, such as the $G^0\partial G^+\,b\bar{t}$ terms induced by the current operator $\Opp{\phi Q}{(3)}$, which leads to maximal $E^2$ growth. This is analogous to the $b\,W\to t\,H$ scattering in the previous section, replacing the dynamical Higgs in Eq.~\eqref{eq:OphiQ3} with a neutral Goldstone boson.
    %One can alternatively think of the growth as arising from the spoiling of the Higgs mechanism that links masses and Higgs couplings of the weak bosons.
% \input{bwtz_table}
\subsection{$\mathbf{t \, h \to t \, h}$ scattering
\label{subsec:thth}
}
    \begin{figure}[h!]
        \centering
        \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/thth_1}
        }  \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/thth_2}
        }
        \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/thth_3}
        }
        \caption{SM diagrams for the $t h \to t h$ subprocess. \label{thth_sm}}
    \end{figure}    
\noindent This process is the simplest in terms of the degrees of freedom involved. The only relevant couplings are the top-Higgs and the triple Higgs interactions (see Fig.~\ref{thth_sm}). Table~\ref{tab:thth}  can be understood in terms of dimension 5 interactions. The operator $\Op{t \phi}$, for example, generates a contact term $tthh$, while the operator $\Op{\phi D}$ a triple Higgs interaction with 2 derivatives. It is not possible to reproduce this behaviour in the AC framework, without the new Lorentz structures for contact terms and higher-derivative couplings.
% \input{thth_table}
\subsection{$\mathbf{t \, Z \to t \, h}$ scattering
\label{subsec:tzth}
}
    \begin{figure}[h!]
        \centering
        \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/tzth_1}
        }  \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/tzth_2}
        }
        \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/tzth_3}
        }
        \caption{SM diagrams for the $t z \to t h$ subprocess. \label{tzth_sm}}
    \end{figure}   
\noindent This process is similar to the previous one, but with a $Z$ boson instead of a Higgs boson. The relevant couplings of the process are the top-Higgs, the top-$Z$ and the $Z$-Higgs (see Fig.~\ref{tzth_sm}). The top-$Z$ coupling is present in every diagram, and therefore does not play a role in unitarity cancellations. We can therefore consider anomalous top-Higgs and $Z$-Higgs couplings to search for energy growth, as previously done for $b \, W \to t \, h$. One can verify that there are 2 helicity configurations, $(-1,0,1,0)$ and $(1,0,-1,0)$ that grow with energy unless the couplings obey relations determined by the Higgs mechanism. The amplitudes are proportional to
    \begin{equation}
        \sqrt{-t}\,(m_t g_{Zh} - 2 m_Z^2 g_{th}) \,,
    \end{equation}
and here are no higher degrees of growth from ACs. This can be reproduced in the SMEFT by means of the Yukawa operator $\Op{t \varphi}$, as for $b\,W\to t\,h$ scattering. An analogous effect arises from the operator $\Op{\varphi D}$ that modifies the $Z$ mass and the coupling of the $Z$ to the Higgs boson. All the other operators in Table~\ref{tab:tzth}  can be related to pure contact terms arising at dimension-6, such as maximal growth observed for the $h\partial G t\bar{t}$ terms induced by the three current operators.
% \input{tzth_table}
\subsection{$\mathbf{t \, Z \to t \, Z}$ scattering
\label{subsec:tztz}
}
    \begin{figure}[h!]
        \centering
        \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/tztz_1}
        }  \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/tztz_2}
        }
        \subfloat[]{
        \includegraphics[width=0.25\linewidth]{Images/tztz_3}
        }
        \caption{SM diagrams for the $t Z \to t Z$ subprocess. \label{tztz_sm}}
    \end{figure} 
\noindent In this process the top-Higgs, the top-$Z$ and the $Z$-Higgs couplings are probed as can be seen in Fig.~\ref{tztz_sm}. None of them are present in every diagram, meaning that they all participate in the SM unitarity cancellation in  the $(-1,0,1,0)$ and $(1,0,-1,0)$ helicity configurations. The amplitudes are proportional to
     \begin{equation}
         \sqrt{-t}\,(\gth \, \gzh - 2 \mt^2 (\gztl-\gztr)^2) \, .
     \end{equation}
There are no higher degrees of energy growth in the AC framework. This behaviour can also be mapped to the SMEFT by means of the operators $\Op{t \varphi}$, $\Op{\varphi D}$, $\Op{\phi Q}^{\sss (3)}$ and $\Op{\varphi t}$ that  modify the aforementioned couplings and/or the top/$Z$ mass.

This process has no contact terms in unitary gauge coming from the dimension 6 operators. In Feynman gauge some contact terms are found involving Goldstone bosons for the dipole operators $\Op{t W}$ and $\Op{t B}$ ($G^0\partial Z\,  t\bar{t}$) but not for the current operators. This is consistent with the lack of maximal energy growth for the corresponding purely longitudinal configurations (see Table~\ref{tab:tztz}). The operators like $\Op{\varphi W}$ modify the coupling of the $Z$ to the Higgs but with an effective dimension 5 vertex that affects only the transverse degrees of freedom of the weak boson.
%
% \input{tztz_table}
%
\subsection{$\mathbf{t \, W \to t \, W}$ scattering
\label{subsec:twtw}
}
\begin{figure}[h!]
        \centering
        \subfloat[]{
        \includegraphics[width=0.24\linewidth]{Images/twtw_1}
        }  \subfloat[]{
        \includegraphics[width=0.24\linewidth]{Images/twtw_2}
        }
        \subfloat[]{
        \includegraphics[width=0.24\linewidth]{Images/twtw_3}
        }
        \subfloat[]{
        \includegraphics[width=0.24\linewidth]{Images/twtw_4}
        }
        \caption{SM diagrams for the $t W \to t W$ subprocess. \label{twtw_sm}}
    \end{figure} 
\noindent This process involves the top-$Z$, top-$\gamma$, triple gauge, top-Higgs,  $W$-Higgs and  weak current couplings to the $W$ (see Fig.~\ref{twtw_sm}). In the SMEFT the SM top coupling to the photon is protected by $U(1)_Q$ and therefore cannot be affected by the operators, only dipole type interactions can be induced for the vertex. In this process there are many unitarity cancellations, involving various combinations of the couplings. One can produce maximal growth proportional to $E^2$ due to additional sources of spontaneous symmetry breaking effects analogous to $b\,W\to t\,Z$ scattering. To show an example, the AC $(-1,0,-1,0)$ helicity configuration is proportional to
    \begin{equation}
        \sqrt{s(s+t)}\,(\gbtw^2 - \gta \, \gwa - \gwz \, \gztl) \,,
    \end{equation}
which  mixes gauge-fermion and gauge self-interactions.
Other helicity amplitudes also exhibit cancellations, some of them involving the gauge couplings and others involving the couplings to the Higgs and the top mass. As discussed previously, the SMEFT cannot explicitly break gauge invariance, but we can map the violations related to the additional sources of spontaneous breaking, either involving Higgs or the Goldstone bosons. Table~\ref{tab:twtw}  can be understood in analogy to the previous processes, in terms of contact terms with Goldstones or dimension-5 effective operators that introduce a new Lorentz structure to Standard Model interactions.
%
% \input{twtw_table}
%
\subsection{Scatterings with photons \label{subsec:photons}}
In this section we discuss the scattering amplitudes involving at least one photon. As mentioned before, the SM photon coupling is protected by the conservation of electric charge, meaning that fewer operators enter in this set of processes. The only possible sources of modified interactions come from new Lorentz structures, such as 
dipoles and triple gauge operator. The tables for the processes are 
given in Tables~\ref{tab:bwta}--\ref{tab:tzta}. The only possible dimension-6 contact terms that could lead to maximal growth are of the $(G/h)\partial V \,f\bar{f}$ type induced by the dipole operators and will contribute to transverse-longitudinal configurations of amplitudes with only one photon. The higher-derivative Lorentz structure of the triple gauge operator $\Op{W}$ is also found to induce maximal energy growth in fully transverse $b\,W\to t\, \gamma $ scattering due to the modification of the $WW\gamma$ vertex. All other configurations have at most a linear energy growth.
% % \subsubsection{$b W \to t \gamma$}
% \input{bwta_table}
% % \subsubsection{$t \gamma \to t \gamma$}
% \input{tata_table}
% % \subsubsection{$t \gamma \to t h$}
% \input{tath_table}
% % \subsubsection*{$t Z \to t \gamma$}
% \input{tzta_table}
% \clearpage
    \subsection{Helicity amplitude summary \label{subsec:helamp_summary}}
Table~\ref{tab:helamp_summary}, gives an overview of the energy growths induced by the set of SMEFT operators under consideration. It reports the maximum possible growth in powers of energy, $E$, that each operator brings to a given subprocess. Additionally, the case where this leads to an energy-growing interference term with the SM is highlighted in red. We see that the maximum degree of growth is with the square of the energy, as expected for dimension-6 operators, and is present on every amplitude with the exception of $t h\to  th $ and $t\gamma\to t\gamma$. Since the overall dimension-6 amplitude must have a mass dimension of 2 to compensate for $c_i/\Lambda^2$, linear energy scalings are also proportional to an EW scale mass-parameter, usually $\mt$ or $\mw$. Concerning individual operators,  the maximum growth is induced by the triple-gauge operator, the weak dipole operators and the four current operators. The energy-growing interference behaviour is limited to the current operators apart from the right-handed charged current one. The interference occurs in the fully-longitudinal configurations for which the SM typically has its maximal (constant) behaviour with energy. The triple-gauge and dipole operators preferentially source transverse gauge bosons and the corresponding SM helicity amplitude in each configuration decreases with energy such that the interference term does not grow in absolute terms. The top Yukawa operator and the remaining bosonic operators are only able to induce a linear growth with energy and never interfere with the SM in the high energy limit. 
    
    \begin{table}[h!]
    \input{summary_table}
    \caption{\label{tab:helamp_summary}
    Maximal energy growths induced by each operator on the set of scattering amplitudes considered. No entry denotes no contribution or no energy growth and the entries highlighted in red denote the fact that the interference between the SMEFT and the SM amplitudes also grows with energy, i.e. that the corresponding SM helicity amplitude is constant with energy.
    }
    \end{table}
    



==> physical_processes.tex <==
Having thoroughly analysed the high energy behaviour of the $2\to2$ amplitudes
involving at least one top quark, we now turn to addressing how this can be probed
by physical processes at collider experiments. We consider whether looking at high-energy EW top processes can improve our understanding 
of the interactions of the EWSB sector. In other words, from a SMEFT perspective, 
what new information/sensitivity on the Wilson coefficients can be obtained from collider 
measurements of such processes. In particular we would like to investigate 
the degree to which the behaviour of the $2\to2$ amplitude is preserved when 
going to $2\to3$ or $2\to4$ processes that could occur at colliders. The broad 
classes of processes that we will study are summarised by the Feynman 
diagrams shown in Figure~\ref{fig:process_diagrams}. Each process contains an EW top $2\to2$ scattering sub-amplitude denoted by the 
blob. 
\begin{figure}[h!]
  \centering
  \subfloat[$t\bar{t}X$\label{fig:ttx_diag}]{
  \includegraphics[width=0.33\linewidth]{Images/ttX}
  }  \subfloat[$tXj$\label{fig:txj_diag}]{
  \includegraphics[width=0.3\linewidth]{Images/tXq}
  }
  \subfloat[$tWX$\label{fig:twx_diag}]{
  \includegraphics[width=0.3\linewidth]{Images/tWX}
  }\\
  \subfloat[$t\bar{t}Xj$\label{fig:ttxj_diag}]{
  \includegraphics[width=0.3\linewidth]{Images/ttXq}
  }
  \subfloat[$t\bar{t}XY$\label{fig:ttxy_diag}]{
  \includegraphics[width=0.3\linewidth]{Images/ttXY}
  }
  \subfloat[VBF\label{fig:VBF_diag}]{
  \includegraphics[width=0.27\linewidth]{Images/VBF}
  }
  \caption{ \label{fig:process_diagrams}
  Schematic Feynman diagrams for collider processes probing EW top scattering. 
  The blobs identify the presence of the $2\to2$ sub-amplitude in the process and 
  the double dashes denote either a Higgs or EW gauge boson final state.}
\end{figure} 


Table~\ref{tab:constraints} displays a clear 
hierarchy between the current sensitivity to the operators with and without 
a top quark field. Although this statement is specific to our choice of basis and 
normalisation, one can intuitively understand that the operators not 
explicitly including a top quark field will generally affect other 
interactions that could be better constrained by EW precision, diboson and Higgs 
measurements. We therefore focus on the sensitivity of these 
processes to the remaining set of operators
\begin{align}
\Op{t\phi}, \Op{tB}, \Op{tW}, \Op{\phi Q}^{\sss(1)}, \Op{\phi Q}^{\sss(3)}, \Op{\phi t}, \Op{\phi tb}.
\end{align}

\input{ewa}

\subsection{Blueprint for the numerical analysis\label{sec:blueprint}}
\begin{figure}[h!]
  \centering \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/pptzw_radar_chart"}
  \caption{Radar plot for the process $p \, p \to t \, Z \, W$ at the 13 TeV LHC. The left and right figures show the impact of each operator, for a Wilson coefficient of 1 TeV$^{-2}$, at linear (absolute value of SM--EFT interference) and quadratic (EFT amplitude squared) level in each Wilson coefficient, relative to the SM EW contribution, $\sigma_{\sss EW}$. When present, the inclusive QCD-induced contribution is also shown. The relative impacts at inclusive level and in a high energy region of phase space are depicted by the blue and red dots, respectively (see main text). The stars denote the corresponding prediction when saturating the individual limits on the coefficients summarised in Table~\ref{tab:constraints}.
 \label{fig:radar_tzw_LHC13}}
\end{figure}
\noindent We will consider the constraining power of these processes, through energy growth, in the 
the High-Luminosity LHC phase as well as at future hadron colliders at 27 and 100 
TeV centre of mass energies and a high energy $e^+e^-$ collider operating at 
380 GeV, 1.5 TeV and 3 TeV. The interference 
and squared contributions of each operator, $\mathcal{O}_i$, are computed relative 
to the pure EW SM contribution, and represented by the ratios $r_i$ and 
$r_{i,i}$ respectively.  The 
relative impact is shown for each relevant operator setting the Wilson coefficient 
to 1 TeV$^{-1}$. The absolute value of the interference contribution is reported. 
In the case where there is a corresponding QCD-induced 
contribution, which does not probe the EW $2\to2$ scatterings, this rate is also 
quoted. We also consider the relative impact of the operator on the EW processes 
when saturating the individual limits quoted in Table~\ref{tab:constraints} to 
give an idea of whether each process may provide additional sensitivity to a 
particular operator given existing constraints. In order to determine the high 
energy behaviour of each process, we compute both the inclusive production cross 
sections and the cross sections in a restricted, high energy region of phase 
space determined by a process dependent cut on a particular kinematical variable. 
A substantial growth in the relative impact of the operator can indicate the 
presence of unitarity violating behaviour due to the effective operator insertions.
In the case of the interference contribution, the assessment is more subtle due 
to the non-positive-definite nature of this term in the matrix element. The sign 
of the matrix element can change over the phase space and result in cancellations 
upon integration. This can result in `anomalously' small contributions 
compared to other, similar operators and obfuscate the high energy behaviour 
present in the EFT contribution to the amplitude. We will identify these occurrences 
in the following survey of processes.

We present the results in a compact format by making use of radar plots of the kind
shown in Fig~\ref{fig:radar_tzw_LHC13}. Whenever a charged particle is present in the final
state we always include contributions for both particle and antiparticle in the numerical
results. The radar plots provide various information. In the top left corner the inclusive
EW and QCD (if present) cross sections for the process are displayed. The bottom left corner shows a list of the 
$2 \to 2$ sub-amplitudes probed. We plot the ratios $r_i$ and $r_{i,i}$ on a logarithmic scale
for each of the selected operators, highlighting the circle corresponding to a $100\%$ relative
contribution to the SM. The blue dots show the value of the ratios at the inclusive level, $r^\text{tot}$, while the
red dots in the high energy region of phase space, $r^\text{HE}$. For the final state $t \, Z \, W$ for example, 
the high energy region is selected with a $p_T > 500$ GeV cut on both weak bosons. The stars
provide information on the attainable sensitivity when the current limits on the Wilson
coefficients are saturated. The shading is added simply as a visual aid. By looking at the radar plot for $t \, Z \, W$ one can 
notice that not only is the process more sensitive to certain operators than
others, but also that the high energy cut enhances some more than others. For example
the constraining power for this process to the Yukawa operator seems feeble,
while the dipoles have a significant impact both at the interference and square level.
A common feature to all processes, clearly noticeable in Fig~\ref{fig:radar_tzw_LHC13},
is the fact that the high energy cut enhances more the square contribution than the
interference, as naively expected by the energy behaviour of the $2 \to 2$ sub-amplitudes. 

In some cases, we consider processes with a light jet in the final state. These are defined {\it excluding} $b$-jets. The main reason behind this is, on one side, that processes with final state $b$'s can be considered experimentally distinct from processes involving gluons or light jets (even though we are technically employing the 5-flavour scheme for our numerical simulations) and on the other, that $b$-quark final states can also introduce dependence on charged $2\to2$ subprocesses, {\it i.e.}, $b W\to t X$, not present in all other channels. These types of processes are therefore also phenomenologically distinct from the perspective on constraining the high energy behaviour of EW top quark scattering.  Notwithstanding the omission of outgoing $b$-quarks, such final states can often be obtained as a real QCD radiation from an underlying Born-level process. These are not infrared finite on their own given that they form a subset of the NLO QCD corrections to said process.  An example of this is $tWj$, which has an order $\alpha_{\sss EW}^3$ contribution related to $b\,W\to t\,Z$ scattering as well as an order $\alpha_{\sss S}^2\alpha_{\sss EW}$ component coming from real QCD corrections to $tW$ production. We can nevertheless study these EW components independently, bearing in mind that they will always have an additional QCD-induced background. When computing predictions for these processes, a suitable jet $p_T$ cut must be applied to avoid the singular phase space region. These cuts are chosen in a process-dependent way, by studying the stability of the ratio between the EW- and QCD-induced versions of the process, choosing a cut for which this ratio has roughly plateaued and the absolute size of the QCD component of the cross section ($tWj$ at $\mathcal{O}(\alpha_{\sss S}^2\alpha_{\sss EW}$))is lower than that of the underlying Born process ($tW$). 

\subsection{$t\bar{t}X$ processes
\label{subsec:ttX}}
The first kind of processes that come to mind for probing the EW interactions 
of the top quark are the associated production of a top quark pair with a EW 
gauge boson or Higgs. The recent discovery of the $t\bar{t}H$ production mode 
means that all of these processes have now been observed at the LHC. 
Concerning sensitivity to the EW 
scattering amplitudes, these processes have the significant drawback of being 
dominantly QCD-induced at hadron colliders through the usual $t\bar{t}$ 
production channels. These do not contain the $2\to2$ sub-amplitudes of 
interest, which are present in the pure EW contribution to this final 
state, typically 2 orders of magnitude smaller than the former. Even though the $2\to2$
scattering amplitudes are not present in the QCD processes, the operators that 
we study can still affect the total rate of these processes by shifting the SM 
couplings of the top quark to the EW gauge bosons or the Higgs, as has been 
studied in Refs.~\cite{Bylund:2016phk,Maltoni:2016yxb}. Therein, a relative impact (of coefficients set to 1 TeV$^{-2}$) on $t\bar{t}Z$ of order 6-10\% is predicted from the current operators coming mainly from the interference term. The dipole interference terms only contributes at the permille level while the squared piece is relatively enhanced and can give an effect of a few percent. $t\bar{t}H$ is analogously affected by $\Op{t\phi}$ at the 10\% level. One 
therefore requires an $\mathcal{O}(10-50)$ enhancement of the EW-induced processes at high energies in order 
to have a visible impact on the total hadron collider rate that competes with the modification of the QCD induced processes. We define our high energy region by imposing a $p_T$ cut of 500 GeV on both the top and the anti-top. Although the aforementioned current and Yukawa operator contributions to $t\bar{t}Z$ and $t\bar{t}H$ respectively will not grow with energy, one should keep in mind that the small dipole operator contributions at inclusive level will be enhanced by said cut. Finally, the EW channels 
generally feature an off-shell, intermediate gauge boson in the $s$-channel that 
introduces an automatic $1/s$ suppression in the amplitude, as seen in Figure~\ref{fig:ttx_diag}. Altogether, these processes 
are not ideal for probing the high energy kinematics of the $2\to2$ sub-amplitudes that we have studied.
We now explicitly verify this for each process in turn.
\subsubsection{$t\bar{t}Z$ \& $t\bar{t}H$
\label{subsubsec:ttZ_ttH}}
At hadron colliders, $t\bar{t}Z$ probes the $t\,Z\to t\,Z$, $t\,Z\to t\,\gamma$ and $b\,W\to t\,Z$
sub amplitudes. The latter enters through the $b\bar{b}$ initiated process 
in which a $W$-boson is exchanged in the $t$-channel. Interestingly, this 
sub-process is found to give the dominant contribution to the EW-induced component 
of $t\bar{t}Z$ production, accounting for nearly 90\% of the total rate at the 13 TeV LHC. 
The PDF suppression of the $b\bar{b}$ luminosity is overcome by the favourable 
$t$-channel kinematics of the process compared to the highly off-shell, $s$-channel 
$Z/\gamma$ contributions. Given than it is a qualitatively different process,  probing an entirely new channel, we start by dropping this contribution and discussing it separately. {\color{green} (Is it discussed somewhere?)} The upper plot of Figure~\ref{fig:radar_ttz_tth_LHC13} summarises the impact of the SMEFT operators on this process 
at the 13 TeV LHC. The non-$b$ induced, pure EW contribution to the cross section is 1.6 
fb, to be compared with 587 fb in the case of the QCD-induced component.
\begin{figure}[h!]
  \centering \includegraphics[height=0.2\paperheight]{"Images/radar_charts_LHC_processes/ppttz_nob_radar_chart"}\\[1.5ex] \includegraphics[height=0.2\paperheight]{"Images/radar_charts_LHC_processes/pptth_nob_radar_chart"}
  \caption{ 
   Radar plot for the $p \, p \to t \, \bar{t} \, Z$ (upper row) and $p \, p \to t \, \bar{t} \, H$ (lower row) processes at the 13 TeV LHC, see
 Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_ttz_tth_LHC13}}
\end{figure}
Although some sensitivity to the operators is present, the required enhancement 
to overcome the large QCD contribution is not observed. In the interference contribution, 
energy growth is essentially absent.
% The current operator, 
%$\Opp{\phi Q}{(3)}$, has an energy-growing interference contribution in the 
%$b\,W\to t\,Z$ sub-amplitude that is not reflected in this process. The 
%$\Opp{\phi Q}{(1)}$ interference term appears to grow with energy due a 
%cancellation over the inclusive phase space that is 
%undone when requiring a high $p_T$ top quark. The inclusive contribution is 
%two orders of magnitude smaller that that of the other current operators while 
%the high-$p_T$ rate is comparable, indicating that a cancellation is likely 
%occurring in the former. 
The interferences of the two quark doublet current operators, $\Opp{\phi Q}{(3)}$ and $\Opp{\phi Q}{(1))}$ have an order 10\% effect while the 
right handed current, $\Op{\phi t}$, and the Yukawa operator, $\Op{t\phi}$ both  have a very mild impact on 
this process. The lack of energy growth in these operator contributions is also present in the quadratic terms, which have a small impact overall. Even when saturating the current limits, the net contribution of these pieces are below those of the interference. The dipole operators could contribute $\mathcal{O}(10)$ effects and display some mild energy growth in their interference which is enhanced at quadratic-level.

The $t\bar{t}H$ process is qualitatively similar to $t\bar{t}Z$ with the 
exception that the Higgs cannot be radiated from the initial state. This results 
in larger relative contributions from the dimension-6 operators. The non-$b$ induced EW cross 
section is only 0.7 fb and competes with 399 fb for the QCD induced process. 
It contains the $t\,Z\to t\,h$, $t\,h\to t\,\gamma$ sub-amplitudes. Once again we observe that nearly 70\% of the 13 TeV LHC rate would in fact be mediated by the $b$-quark initial state that probes the charged $b\,W\to t\,h$ channel. 
Table~\ref{tab:helamp_summary} suggests that an interfering energy growth from 
the current operators may be present through $t\,Z\to t\,h$ scattering. 
Figure~\ref{fig:radar_ttz_tth_LHC13} shows that the relative impact of each 
operator is more pronounced than for $t\bar{t}Z$, with the dipole operators in particular yielding $\mathcal{O}(1-10)$ effects at inclusive level that grow by a factor of ten at high energies. A mild growth is confirmed in the interference from the current operators. Sensitivity to the Yukawa operator is also increased with respect to $t\bar{t}Z$ although no growth with energy is observed. A cancellation in the $\Op{\phi t}$ interference contribution is present upon making the high energy cut. Setting the coefficients to their limit values confirms that the required enhancements to overcome the QCD-induced process are not possible, except in the case of the weak dipole operators that could provide as much as a 100-fold enhancement of the EW contribution already at inclusive level. 
\subsubsection{$t\bar{t}W$
\label{subsubsec:ttW}}
The $ttW$ process is somewhat unique in that the corresponding QCD induced process cannot probe modified EW interactions in the top sector since the $W$ boson is uniquely emitted from the initial state quark leg. In the EW case, only the $tW\to tW$ sub-amplitude is accessed, where a $W$-boson is produced in the s-channel and subsequently emits a Higgs or $Z$ boson that splits into the $t\bar{t}$ final state. Figure~\ref{fig:radar_ttw_LHC13}, shows that all operators contribute at or below the 10\% level for $c_i=1$ apart from $\Op{tW}$ that can produce $O(1)$ effects. No energy growth is observed at interference level and the effects at squared level for the current operators is very mild, while some limited growth is present in the case of the weak dipole operators. Combined with the fact that the QCD induced contribution is $\mathcal{O}(100)$ times bigger than the EW one (354 vs. 2.9 fb), this process is not likely to be among the most interesting candidates for probing high energy EW scatterings of top quarks. We will see that the $ttWj$ process is a more favourable environment for accessing this scattering.
\begin{figure}[h!]
  \centering \includegraphics[height=0.2\paperheight]{"Images/radar_charts_LHC_processes/ppttw_radar_chart"}
  \caption{ 
   Radar plot for the $p \, p \to t \, \bar{t} \, W$ process at the 13 TeV LHC, 
 , see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_ttw_LHC13}}
\end{figure}
\subsubsection{$t\bar{t}\gamma$}
The QCD induced $t\bar{t}\gamma$ cross section is estimated to be of the order of  2 pb which , similarly to $t\bar{t}Z$ and $t\bar{t}H$, is about 100 times larger than the EW component that embeds the $t\,Z\to t\,\gamma$ and  $t\,\gamma\to t\,\gamma$ scatterings.  As discussed in Section~\ref{subsec:photons}, as far as top quark operators go, the scatterings only provide sensitivity to one linear combination of the dipole operators, with maximal growth only possible in the transverse-longitudinal configuration of $t\,Z\to t\,\gamma$. Refs.~\cite{Bylund:2016phk} reports sub-percent effects on the QCD-induced inclusive cross section, meaning that an $\mathcal{O}(1)$ impact on the EW component from the dipole operators would be competitive. However, we see in Figure~\ref{fig:radar_tta_LHC13} that the effect is about an order of magnitude too small. As expected it displays some growth with energy which is not as valuable given that the same operator contributions to the QCD-induced process will also do so.

\begin{figure}[h!]
  \centering  \includegraphics[height=0.2\paperheight]{"Images/radar_charts_LHC_processes/pptta_radar_chart"}
  \caption{ 
    Radar plot for the $p \, p \to t \, \bar{t} \, \gamma$ process at the 13 TeV LHC, 
 see
   Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_tta_LHC13}}
\end{figure}
\subsection{Single-top processes
\label{subsec:singletop}}
Single-top processes are a natural candidate for probing the scattering amplitudes of interest. Firstly, the presence of only one top quark guarantees that the process will contain EW interactions at born-level and at most a single QCD vertex coming from an initial state gluon. Consequently, the $2\to 2$ EW scattering amplitudes are present in the leading contribution to such processes and furthermore, are not accompanied by an off-shell $s$-channel resonance that could damp the energy growth as in the $t\bar{t}X$ processes discussed in the previous section. The processes can be categorised in terms of the corresponding single-top production channel, which are the `mother' processes of those that we consider here. They therefore necessarily probe the charged EW scatterings involving both a top and a $b$-quark (and consequently a $W$ boson). For these processes, we impose a $p_T$ requirement of 500 GeV on both the top quark and the associated boson to access the high energy region. 

\subsubsection{$tZj$ \& $tHj$
\label{subsubsec:tZj_tHj}}
These two processes arise from the additional emission of a $Z$ or Higgs boson from the $t$-channel single-top process (see Figure~\ref{fig:txj_diag}). The high energy behaviour of these processes was studied with respect to the $2\to 2$ scatterings in a preliminary way in Ref.~\cite{Degrande:2018fog}. Similarly to the case of $t\bar{t}Z$ and $t\bar{t}H$, $tZj$ admits the radiation of the $Z$-boson from any of the four fermion legs, while $tHj$ is limited to the emission of the Higgs boson from the top quark. The latter is therefore an especially clean probe of the EW scatterings as they as necessarily present in every diagram. This is the reason why it was chosen as the example process to study in the EWA in Section~\ref{sec:EWA}. Therein, we learned that the energy growth of the $2\to 2$ scatterings is definitely present in the parts of phase space in which the approximation holds. The results for the full process that we will show will allow us to ascertain whether this region of phase space is effectively accessed when making some high energy cuts. 

$tZj$ is by far the most abundant of the two processes with an inclusive cross section of order 600 $fb$. Evidence for this process has recently been observed for the first time at the LHC~\cite{Aaboud:2017ylb,CMS-PAS-TOP-16-020,Sirunyan:2017nbr}. The corresponding $b\,W\to t\,Z$ subprocess is sensitive to 6 of the 7 operators that we study in detail here, with the exception of the Yukawa operator. The upper plot of Figure~\ref{fig:radar_tzj_thj_LHC13} reports our results for the 13 TeV LHC in the operator space. The energy-growing interference contribution expected for $\Opp{\phi Q}{(3)}$ is not observed at inclusive level. Subsequent investigation showed that the cross section for the production of purely longitudinal $Z$ bosons revealed the expected energy growing interference, suggesting that the full process is dominated by the transverse modes, even after the high-energy cut. The only significant high energy behaviour to be noted at interference level is the behaviour of $\Op{tW}$, that displays a huge energy enhancement suggestive of a cancellation at inclusive level. The neutral current operators show a milder energy growth, as expected, with the right handed $\Op{\phi t}$ even displaying a decrease with energy. The squared contributions from the SMEFT operators, however, exhibit the strong growth with energy in line with the expectations from the $2 \to 2$ computations. The operators that mediate a $G^+\partial G^0\,\bar{t}b$ contact interaction, $\Opp{\phi Q}{(3)}$ and $\Op{\phi tb}$, grow significantly, as do the dipoles, while the two other contact operators show slightly less pronounced but nonetheless significant growth. The relatively large cross section of this process will most likely permit certain differential measurements to be performed that could provide access to the high energy behaviour of the EW sub-amplitudes. 

As seen in the the lower panel of Figure~\ref{fig:radar_tzj_thj_LHC13}, the $tHj$ process, on the other hand, displays an apparent growth at interference level for $\Opp{\phi Q}{(3)}$. This is, in fact, enhanced by a cancellation at inclusive level which is consistent with the fact that the absolute size of the inclusive interference piece (blue dot, lower left plot) is smaller than the squared one (blue dot, lower right plot). Although this is a normalisation dependent statement for a given process, comparison to other processes such as $tZj$ or $tZW$ (Figure~\ref{fig:radar_tzw_LHC13}) show that this relative suppression is not universal and therefore indicates the presence of a cancellation in $tHj$. We also observe a very strong dependence on $\Op{tW}$, that grows with energy already at the interference level. Saturating the limits on this coefficient still produce $O(5)$ effects on the inclusive rate, meaning that the measurement of this process at the LHC would considerably improve the current constraints on this operator. Finally, sensitivity to the Yukawa is found with $O(1)$ effects incurred when saturating existing limits. Considerable energy growth is found from the unitarity violating behaviour discussed in Section~\ref{sec:bwth}. As discussed in  Ref.~\cite{Degrande:2018fog}, the relatively small cross-section coupled with the challenging final state means that it is unlikely that this process will be accessed at differential level. The inclusive measurement of this channel and the differential measurement of the $tZj$ counterpart are therefore argued to be complementary ways to access the operators that we consider.
\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/pptzj_radar_chart"}\\[1.5ex]
    \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/ppthj_radar_chart"}
  \caption{ 
    Radar plot for the $p \, p \to t \, Z \, j$ (upper row) and $p \, p \to t \, H \, j$ (lower row) processes at the 13 TeV LHC, see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main textSection~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_tzj_thj_LHC13}}
\end{figure} 
% \subsubsection{}
% \begin{figure}[h!]
%   \centering
%
%   \caption{ \label{fig:radar_thj_LHC13}}
% \end{figure}
\subsubsection{$t\gamma j$
\label{subsubsec:taj}}
This process has a significantly larger cross section than $tZj$ and probes $b\,W\to t\,\gamma$ scattering. Figure~\ref{fig:radar_taj_LHC13} shows that the cancellation at inclusive level observed in $tZj$ from $\Op{tW}$ is also not present, instead appearing to affect the  $\Op{tB}$ contribution. Some energy growth is also present, particularly at squared level.
\begin{figure}[h!]
  \centering \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/pptaj_radar_chart"}
  \caption{ 
    Radar plot for the $p \, p \to t \, \gamma \, j$ process at the 13 TeV LHC, see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_taj_LHC13}}
\end{figure} 
\subsubsection{$tZW$ \& $tHW$
\label{subsubsec:tZW_tHW}}
These two processes, in analogy with $tZj$ and $tHj$ to $t$-channel single-top, arise from the additional emission of a $Z$ or Higgs boson from the $tW$ single-top process (see Figure~\ref{fig:twx_diag}). They are sensitive to the same sub-amplitudes as their $t$-channel counterparts. The relative smallness of $tW$ compared to $t$-channel single-top production is propagated to the relative rates of $t(Z/H)j$ and $t(Z/H)W$. One important difference between the two sets of processes, however, is the fact that the bosons participating in the $2\to 2$ scattering are both in the final state in $tZW$ and $tHW$. This means that their polarisation can in principle be measured. The contribution of each polarisation to the full $2\to3$ rate is separate and does not depend on its interaction with the light quark current, in contrast to $tZj$ and $tHj$ (see the EWA discussion of Section~\ref{sec:EWA}). A significant experimental caveat, however, is the similarity of the $tXW$ final state to that of $t\bar{t}X$. After decaying the top quarks, the two only differ by a single $b$-quark. This is conceptually identical to the overlap between the $tW$ and $t\bar{t}$ final states. It may be experimentally challenging to distinguish the two processes, the latter of which has much larger cross section owing to the QCD-induced component. However, the fact that evidence for the $tW$ single-top channel was observed already at 7 TeV gives us hope that $tXW$ is not out of reach at the LHC.

This study has revealed $tZW$ production to be a particularly interesting candidate for probing the high energy behaviour of $b\,W\to t\,Z$ scattering. Figure~\ref{fig:radar_tzw_LHC13}, shown earlier in Section~\ref{sec:blueprint}, 
demonstrates a clear improvement of inclusive sensitivity and energy growth compared to $tZj$ (Figure~\ref{fig:radar_tzj_thj_LHC13}), across the board. The process exhibits the expected energy growth at interference level for $\Opp{\phi Q}{(3)}$, without any evidence of a cancellation. The cancellation of the $\Op{tW}$ interference term in the inclusive cross section is also not present, leading to an improved overall sensitivity. The energy growth observed for this term is not naively expected from the $2\to 2$ analysis. There does, however, appear to be a cancellation in the inclusive $\Op{tB}$ interference contribution.  The energy growth of the squared terms is an enhanced version of the $tZj$ process. From a theoretical perspective, we find this process to be extremely promising. On a practical level, the corresponding cross section is about five times smaller than $tZj$, meaning that it may take more time to observe this process and the possibility of differential measurements is yet unclear. Overall, we conclude that it would be very valuable in the context of globally constraining the SMEFT in the top sector to take on the challenge of measuring this process and distinguishing it from $t\bar{t}Z$.

Interestingly, from a sensitivity perspective,  $tHW$ does not appear superior to $tHj$ in the way that $tZW$ is to $tZj$. Figure~\ref{fig:radar_thw_LHC13} displays a slightly milder sensitivity to the set of operators entering in $b\,W\to t\,h$, with the exception of the absence of a cancellation in the $\Opp{\phi Q}{(3)}$ interference term for the inclusive rate. The global energy growing behaviour is analogous to $tHj$ and, given that the total cross section is even smaller, we conclude that this process is not likely to be isolated at the LHC and therefore is not an interesting production mechanism to study in the SMEFT context.
\begin{figure}[h!]
  \centering \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/ppthw_radar_chart"}
  \caption{ 
    Radar plot for the $p \, p \to t \, H \, W$ process at the 13 TeV LHC, see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_thw_LHC13}}
\end{figure} 
\subsubsection{$tWj$
\label{subsubsec:tWj}}
$tWj$ can be considered a `hybrid' between the $t$-channel and $tW$ single-top production mechanisms. On one hand, the purely EW induced process is similar to the $tZj$ processes, simply interchanging the virtual and final state gauge bosons and has a cross section around 1 pb. On the other, it has a significant QCD-induced component arising due to real radiation from $tW$ production, which we compute to be of order 20 pb for a jet $p_T$ cut of 40 GeV. Furthermore, and perhaps crucially, the $tWj$ final state only differs after top decay from $t\bar{t}$ by a single $b$-tag. A $t\bar{t}$ event with one $b$-quark mis-tagged as a light jet would have an identical final state to $tWj$, suggesting that significant kinematical discrimination techniques would have to be employed to isolate the EW component of this process. 

Concerning EW sub-amplitudes, $tWj$ contains both the $bW\to tZ$ and $bW\to t\gamma$ scatterings. As shown in Figure~\ref{fig:radar_twj_LHC13}, it exhibits a similar, slightly milder, sensitivity profile to $tZj$ and $tZW$. Here the strong cancellation in the $\Op{tW}$ interference contributions is again not present and some energy growth in the interference of $\Opp{\phi Q}{(1)}$ and $\Opp{\phi Q}{(3)}$ is observed. Overall, this process may provide some useful information in a global SMEFT fit, assuming one is able to disentangle it from $tW$ and $t\bar{t}$.
\begin{figure}[h!]
  \centering \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/pptwj_radar_chart"}
  \caption{ 
    Radar plot for the $p \, p \to t \, W \, j$ process at the 13 TeV LHC, see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_twj_LHC13}}
\end{figure} 

\subsection{$t\bar{t}Xj$ processes
\label{subsec:ttXj}}
As discussed in Section~\ref{subsec:ttX}, the $t\bar{t}X$ processes suffer from several drawbacks when in comes to accessing the high energy regime of EW scattering processes contained within. One way to remove the off-shell, $s$-channel topology of these processes is to require the presence of an additional jet, as shown in Figure~\ref{fig:ttxj_diag}. This topology effectively turns the $t\bar{t}X$ diagram (Figure~\ref{fig:ttx_diag}) on its side, and connects the top quark line to an initial state gluon. We will see that these types of processes are much more sensitive to the high energy scattering sub-amplitudes. Concerning the QCD-induced counterparts, we are again in the situation where the $t\bar{t}Xj$ corresponds to a real radiation correction to the born-level $t\bar{t}X$ process. The high energy region here is obtained by imposing a 500 GeV $p_T$ cut on the $X$ boson as well as requiring that only one of either the top or anti-top had a $p_T$ greater than 500 GeV. This seemingly contrived cut is a result of the fact that either top or the anti-top can `participate' in the hard $2 \to 2$ sub-amplitude in this topology.
\subsubsection{$t\bar{t}Wj$
\label{subsubsec:ttWj}}
Section~\ref{subsubsec:ttW} highlights the fact that the $t\bar{t}W$ process is not ideal for probing our top quark operators in  $t\,W\to t\,W$ scattering. Figure~\ref{fig:radar_ttwj_LHC13} shows a clear improvement in sensitivity over the former (Figure~\ref{fig:radar_ttw_LHC13}) with inclusive contributions of up to order one when saturating the limits. A key change is the 20-fold improvement in the relative size of the pure EW and QCD-induced contributions from a factor 100 to a factor 5, meaning that the EW component of around 50 $fb$ is distinctly more accessible in this case. Although the relative impact at inclusive level is not significantly improved, even decreasing slightly in some cases, more energy growing behaviour is present.
\red {At interference-level, $\Opp{\phi Q}{(1)}$, $\Op{tW}$ and $\Op{t \phi}$ display signs of growth while a cancellation with increasing energy causes a decrease in the $\Opp{\phi Q}{(3)}$ and  $\Op{\phi t}$ terms which are expected to grow in the fully longitudinal $t\,W\to t\,W$ helicity amplitude. $\Op{tB}$ also displays a decrease with energy which could be due to the fact that the maximum energy growth of the $2\to 2$ sub-amplitude is proportional to E compared to the E$^2$ dependence of the $\Op{tW}$ contribution. The squared SMEFT contributions, however, display a strong growth with energy. This is consistent with the previous study of this channel in Ref.~\cite{Dror:2015nkp}, which identified it as a promising avenue for the measurement of $tW$-scattering. }
\begin{figure}[h!]
  \centering \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/ppttwj_excut_radar_chart"}
  \caption{ 
    Radar plot for the $p \, p \to t \,\bar{t}\, W \, j$ process at the 13 TeV LHC, see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_ttwj_LHC13}}
\end{figure} 
\subsubsection{$t\bar{t}Zj$ \& $t\bar{t}Hj$
\label{subsubsec:ttZj_ttHj}}
The neutral counterparts of $t\bar{t}Wj$ probe the complementary set of neutral EW scattering amplitudes. We observe an enhancement of a factor of around 4 with respect to the EW $t\bar{t}(Z/h)$ to $t\bar{t}(Z/H)j$ at inclusive level.
The relative size of the EW and QCD contributions, as defined by our jet $p_T$ cut, improves by a factor for about 5 in both cases. Interestingly, this difference is not as striking as in the case of $t\bar{t}Wj$ whose EW contribution seems to benefit from a peculiar enhancement with the addition of one jet in the final state. \red{Why?}. In analogy with $t\bar{t}Z(H)$, the QCD piece also receives similar, energy-constant contributions from the current(Yukawa) operators. The required enhancement of the EW amplitudes in order to compete with these modifications is relaxed to the order of a few.
The `strong scattering' contribution to $ttZj$ depicted in Figure~\ref{fig:ttxj_diag} contains the $t\,Z\to t\,Z$ and $t\,Z\to t\,\gamma$ sub-amplitudes, and analogously contains $t\,h\to t\,Z$ and $t\,h\to t\,\gamma$ for $ttHj$. As with $tt(H/Z)$, the charged scattering also enters through gluon emission contributions to the $b\bar{b}$ mediated channel. However, this contribution is now small due to the absence of the off-shell $s$-channel suppression of $t\bar{t}X$ discussed in Section~\ref{subsubsec:ttZ_ttH}. It goes from contributing to 90\% of $t\bar{t}Z$ to less than 10\% of the $t\bar{t}Zj$ rate and from 70\% to below 5\% in the $t\bar{t}H(j)$ mode.

Sensitivity-wise, we observe slightly better, $\mathcal{O}(10\%)$ effects on the inclusive rates at interference-level for the current operators in both processes. The interfering energy growth from these operators expected in the $t\,Z\to t\,H$ amplitude is not revealed by the high-energy cut on $ttHj$. The Yukawa and dipole operators affect both processes, $ttHj$ slightly more, the latter having a mild interfering energy growth. In the quadratic contributions, the impact of every operator is enhanced with respect to $t\bar{t}X$, in some cases already at inclusive level. One can also notice the remnant dependence on the $b$-initiated contributions in the mild quadratic dependence on $\Op{\phi tb}$. Furthermore strong energy growth is present in all cases. Considering current limits on the operators, one expects $\mathcal{O}(0.1-1)$ effects to $t\bar{t}Zj$ and $\mathcal{O}(1-10)$ enhancements of $t\bar{t}Hj$ in the current operators, which begin to compete with the corresponding modifications of the QCD-induced piece. The dipoles, however could contribute extreme enhancements, about ten times bigger than the current operators. Saturating the limit on $\Op{tB}$, for example, enhances the $t\bar{t}Hj$ rate by a factor 100, making it as large as the SM QCD component. Now that $t\bar{t}Z$ and $H$ have been measured at the LHC, it may be interesting to consider the impact of exclusive jet multiplicity measurements, particularly in the forward region, to constrain these effects.

\begin{figure}[h!]
  \centering \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/ppttzj_excut_radar_chart"}\\[1.5ex] \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/pptthj_excut_radar_chart"}
  \caption{ 
    Radar plot for the $p \, p \to t \,\bar{t}\, Z \, j$ (upper row) and $p \, p \to t \,\bar{t}\, H \, j$ (lower row) processes at the 13 TeV LHC, see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_ttzj_tthj_LHC13}}
\end{figure} 

\subsubsection{$t\bar{t}\gamma j$}
\begin{figure}[h!]
  \centering \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/ppttaj_radar_chart"}
  \caption{ 
    Radar plot for the $p \, p \to t \,\bar{t}\, \gamma \, j$ process at the 13 TeV LHC, see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_ttaj_LHC13}}
\end{figure} 
\subsection{$t\bar{t}XY$ processes
\label{subsec:ttXY}}
An alternative to requiring an additional jet to attempt to enhance the EW contribution to $t\bar{t}X$ processes is to directly produce an additional EW boson. In doing so, one promotes the QCD-induced component into and EW process that probes the sub-amplitudes of interest. The $gg$-channel mediates a class of diagrams as depicted by Figure~\ref{fig:ttxy_diag} that contain the neutral EW-top $2\to2$ scatterings in a $t$-channel, ladder topology. A nice feature is that each process probes a single sub-amplitude and the invariant mass of the two bosons in the final state is a proxy for the centre of mass energy. Specifically, we require a $p_T$ cut of 500 GeV on each of these particles in order to attempt to access the large $s,-t$ limit of this scattering. \red{The phase space region for quasi on-shell intermediate top quarks also requires that the final state tops be produced in the forward direction.} These processes, however, suffer from very small cross sections due to lack of phase space given that the threshold energies start above 500 GeV. It will be challenging for the LHC to gather sufficient statistics to measure these processes. We therefore show results for a future proton collider at 27 TeV.
\subsubsection{$t\bar{t}ZZ$, $t\bar{t}ZH$ \& $t\bar{t}HH$}
At 13 TeV, the $gg$-channel accounts for a little over half of the $t\bar{t}ZH$ and $t\bar{t}HH$ and third of the $t\bar{t}ZZ$ inclusive rates, which at 27 TeV increases to two thirds and one half respectively. The 13 TeV cross sections are of the order of 1 fb, which prompts us to present predictions for 27 TeV. Table~\ref{tab:helamp_summary} shows that, of the $2\to 2$ scatterings probed by these processes, $t\,Z \to t\,H$ has the most potential for energy growth with maximal and interfering behaviour across the current operators while $t\,Z\to t\,Z$ shows a mild, non-interfering energy growth. $t\,H\to t\,H$ only depends on $\Op{t\phi}$ and grows mildly with energy and we therefore do not show a corresponding radar chart for $t\bar{t}HH$. Figure~\ref{fig:radar_ttzz_ttzh_tthh_LHC27} shows that even at 27 TeV, $t\bar{t}ZH$ and $t\bar{t}ZZ$ have relatively small cross section of around 8-9 fb, with $t\bar{t}HH$ slightly lower at 4.5 fb. Given the similar $t\bar{t}ZH$ and $t\bar{t}ZZ$ rates, one expects the former to provide the most interesting sensitivity. 

Comparing the interference contributions in both processes, one sees that the operators can have an impact of around 10\% in each case, with a slightly better sensitivity for  $t\bar{t}ZH$. Energy growth is, however, not observed to be significant. This is expected for $t\bar{t}ZZ$ but not for $t\bar{t}ZH$ where only the $\Op{\phi t}$ contributions shows some evidence of the expected behaviour. The other current operators display phase space cancellations which is evidenced by a sign change of the interference contributions with increasing $p_T$ cuts. This is shown in Figures~\ref{fig:summary_plot_a3phidql} and~\ref{fig:summary_plot_aphidql}, where the impact with even higher energy cut, not shown in Figure~\ref{fig:radar_ttzz_ttzh_tthh_LHC27} is plotted.

Considering the impact at quadratic-level, however reveals a totally different picture, in which the sensitivity of $t\bar{t}ZH$ is significantly enhanced, especially in its energy growth, while that of  $t\bar{t}ZZ$ is reduced. This is indicative of a phase space cancellation in the interference terms of $t\bar{t}ZH$, given the sudden increase at quadratic level. Indeed we observe that, in increasing the high energy cut, the interference contributions of the current operators do in fact grow with energy but also change sign in the process. For $t\bar{t}ZZ$, in contrast, the relative impact of these terms remains constant. This is consistent with our expectations from the sub-amplitude analysis. Saturating the limits predicts $\mathcal{O}(1$--$10)$ and $\mathcal{O}(0.1$--$1)$ effects on the inclusive $t\bar{t}ZH$ and  $t\bar{t}ZZ$ rates respectively. The Yukawa operator is found to have a $\sim 30\%$ negative impact on the $t\bar{t}HH$ cross section with a mild energy growth only at quadratic level. 
% \begin{figure}[h!]
%   \centering \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/ppttzz_radar_chart"}\\[1.5ex] \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/ppttzh_radar_chart"}% \\[1.5ex] \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/pptthh_radar_chart"}
%   \caption{ \label{fig:radar_ttzz_ttzh_tthh_LHC13}}
% \end{figure}
\begin{figure}[h!]
  \centering \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes_27/ppttzz_radar_chart_27"}\\[1.5ex] \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes_27/ppttzh_radar_chart_27"}% \\[1.5ex] \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes_27/pptthh_radar_chart_27"}
  \caption{ 
    Radar plot for the $p \, p \to t \,\bar{t}\, Z \, Z$ (upper row) and $p \, p \to t \,\bar{t}\, Z \, H$ (lower row) processes at the 27 TeV LHC, see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_ttzz_ttzh_tthh_LHC27}}
\end{figure} 
\subsubsection{$t\bar{t}WW$}
The $gg$-initiated $t\bar{t}WW$ cross section evolves similarly to the previous processes with collider energy, contributing at one half of the total at 13 TeV and two thirds at 27 TeV. The rates are significantly larger than those of the previous section: 8 and 53 fb at 13 and 27 TeV respectively. However, as shown in Figure~\ref{fig:radar_ttww_LHC13_LHC27}, the relative sensitivity at inclusive level is not so strong, contributing 1-10\% effects in the interference terms with evidence of phase space cancellations in dipole and $\Op{\phi t}$  operators. Saturating the limits, one can expect total contributions at most of order one. Energy growth in this channel is quite pronounced, close to that of the $t\bar{t}ZH$ process. Given the much larger rate, one can expect this channel to be an interesting probe of strong EW-scattering at future colliders, particularly if the high energy region is accessed by differential measurements. 
\begin{figure}[h!]
  \centering \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/ppttww_radar_chart"}\\
%   \caption{ \label{fig:radar_ttww_LHC13}}
% \end{figure}
% \begin{figure}[h!]
%   \centering
\includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes_27/ppttww_radar_chart_27"}
  \caption{ 
    Radar plot for the $p \, p \to t \,\bar{t}\, W^+ \, W^-$ processes at the 13 (upper row) and 27 (lower row) TeV LHC, see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_ttww_LHC13_LHC27}}
\end{figure} 
\subsection{Vector boson fusion processes
\label{subsec:VBF}}
The final set of processes we consider are those that produce $t\bar{t}$ in the VBF topology, that is to say in association with a pair of very forward, light fermions. At the LHC these could be any combination of light quarks in the proton. The major drawback of this channel at the LHC is the overwhelming $t\bar{t}$+jets QCD background which, without any selection requirements, has a cross section 5 orders of magnitude larger than the EW process of interest. It is therefore interesting in this case to consider such a production channel at a future high-energy $e^+e^-$ collider, since the initial and final state light fermions need only to have EW interactions. The lack of the aforementioned QCD background coupled with clean environment of such colliders makes them an ideal testing ground for these processes. Additionally, one can distinguish the fusion of neutral and charged EW gauge bosons by whether we observe neutrinos (missing energy) or electrons in the final state. One however requires significant centre of mass energies to access these types of processes. We therefore choose the CLIC accelerator as a benchmark lepton collider to assess the VBF processes, considering the three proposed centre-of-mass energy configurations of 380, 1500 and 3000 GeV. In order to suppress unwanted contributions from on-shell $t\bar{t}(Z/W)$ where the gauge boson decays to a pair of jets or leptons, we require an invariant mass above 100 GeV for the light fermion pair. Analogously to the $t\bar{t}XY$ processes, 500 GeV $p_T$ cuts are imposed on the top quarks to define the high energy LHC cross section. In the case of CLIC, the lowest energy setup is barely in threshold for this process, meaning that high energy cuts cannot meaningfully be imposed. For the 1500 and 3000 GeV cases, we impose top $p_T$ cuts of 1000 and 1500 GeV respectively. 
\subsubsection{$t\bar{t}jj$}
We begin with the proton-proton collider prediction, whose EW component has a cross section of 5.2 fb at 13 TeV. The VBF $t\bar{t}$ component of this process probes a mixture of all neutral $2\to2$ subprocesses not involving the Higgs, which cannot couple to the light quark lines. The charged subprocesses are contained in this final state but are not of the same VBF topology and also enter at the price of a $b$-quark PDF. Of the relevant neutral subprocesses, $t\,W\to t\,W$ is expected to provide the strongest energy growth. Figure~\ref{fig:radar_ttjj_LHC13} shows that only $\Op{\phi t}$ and $\Op{tW}$ display significant energy growth at interference-level. The quadratic contributions do display the expected growth, although their relative impact is mild, giving $O(1)$ effects in the high energy region. The only exception is $\Op{tW}$, that provides an $O(1)$ effect on the inclusive rate that grows by a factor of 10 at high energies. Given the overwhelming QCD background, we do not consider these effects on the EW cross section to be sufficient for VBF $t\bar{t}$ production to yield meaningful additional constraints on the Wilson coefficient space. {\color{green} The QCD number is missing in the radar plot, did we decide to not compute it for some reason that I cannot remember?} \red{I think we decided not to do it at the time as it is just so huge compared to VBF.}
\begin{figure}[h!]
  \centering \includegraphics[width=\linewidth]{"Images/radar_charts_LHC_processes/ppttjj_radar_chart"}
  \caption{ 
    Radar plot for the VBF $t\bar{t}$ production process at the 13 TeV LHC, see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_ttjj_LHC13}}
\end{figure} 

\subsubsection{$t\bar{t}\nu_e\bar{\nu}_e$ \& $t\bar{t}e^+e^-$}
High energy lepton colliders appear to be the most promising avenue for measuring the VBF $t\bar{t}$ process, simply due to the absence of the QCD $t\bar{t}$+jets background. The final state fermions determine whether the dominant VBF contribution comes from the $2\to2$ subamplitudes involving neutral gauge bosons ($e^+e^-$) or $t\,W\to t\,W$ scattering ($\nu_e\bar{\nu}_e$). The non-VBF contributions from $t\bar{t}(Z\to\bar{\nu}_e\nu_e)$ introduce a weak dependence of the latter process on the neutral gauge bosons scatterings ($t\,Z\to t\,Z$ and $t\,Z\to t\,\gamma$) that is negligible compared to $t\,W\to t\,W$. The scatterings involving only neutral gauge bosons have a weaker expected energy dependence than $t\,W\to t\,W$. Combining this with the larger predicted cross sections for  $t\bar{t}\nu_e\bar{\nu}_e$  reported in Figure~\ref{fig:radar_ttvv_CLIC} compared to those of Figure~\ref{fig:radar_ttee_CLIC} leads to a clear preference for this process in constraining SMEFT operators at high energies. Indeed, the figures show qualitatively similar inclusive sensitivities ($O(0.1-1)$) to the 6 operators, with only the hypercharge dipole operator, $\Op{tB}$, having a greater relative impact in $t\bar{t}e^+e^-$. There is evidence for a cancellation in the interference contribution from this operator in $t\bar{t}\bar{\nu}_e\nu_e$. Concerning the high energy behaviour, the expected enhancements from the $t\,W\to t\,W$ scattering are plain to see with the $WW$-fusion process showing larger enhancements both at interference and squared level. That said, the energy growth of the interference terms is somewhat mild, given the expectation of a maximal effect from the current operators in the fully longitudinal $t\,W\to t\,W$ scattering. 
\begin{figure}[h!]
  \centering \includegraphics[width=\linewidth]{"Images/radar_charts_CLIC_380/eettveve_radar_chart_380"}\\[1.5ex]
  \includegraphics[width=\linewidth]{"Images/radar_charts_CLIC_1500/eettveve_radar_chart_1500"}\\[1.5ex]
  \includegraphics[width=\linewidth]{"Images/radar_charts_CLIC_3000/eettveve_radar_chart_3000"}
  \caption{ 
   Radar plot for the $e^+\,e^- \to t\,\bar{t}\,\nu_e\,\bar{\nu}_e$ process at collider centre of mass energies of 380 (upper row), 1500 (middle row) and 3000 GeV (lower row), see
 Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description. 
 \label{fig:radar_ttvv_CLIC}}
\end{figure} 
\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{"Images/radar_charts_CLIC_380/eettee_radar_chart_380"}\\[1.5ex]
  \includegraphics[width=\linewidth]{"Images/radar_charts_CLIC_1500/eettee_radar_chart_1500"}\\[1.5ex]
  \includegraphics[width=\linewidth]{"Images/radar_charts_CLIC_3000/eettee_radar_chart_3000"}
  \caption{ 
    Radar plot for the $e^+\,e^- \to t\,\bar{t}\,e^+\,e^-$ process at collider centre of mass energies of 380 (upper row), 1500 (middle row) and 3000 GeV (lower row), see
  Figure.~\ref{fig:radar_tzw_LHC13} and Section~\ref{sec:blueprint} of the main text for a detailed description.
  \label{fig:radar_ttee_CLIC}}
\end{figure} 

\subsection{Summary}
Our survey of collider processes contains a great deal of information for which a comprehensive synthesis is difficult to provide. We have presented the absolute relative impacts of the operators of interest to a large number of EW processes at both $pp$ and $e^+e^-$ colliders whose SM predictions span several orders of magnitude in cross section. These numbers can serve as a guide for the future directions of top quark measurements targeting SMEFT or modified top-EW interactions in general. However, a number of process-dependent factors must also be taken into account beyond the sensitivity of the EW process, as we have discussed in the individual sections. We have not presented any detailed phenomenological analyses, leaving these for future work. Rather, we have focused on isolating energy growth from the $2\to2$ subamplitudes in the processes relevant for current and future collider searches. 

%
The presence of an irreducible, QCD-induced background which does not embed the $2\to2$ amplitudes is often a `diluting' factor to the sensitivity. In processes with an outgoing light jet, the same final state can be obtained by real QCD radiation from an underlying process, i.e. as part of as NLO QCD correction. 
Furthermore, in some cases the modified SM interactions may also contribute to the overall normalisation of the QCD process, without energy growth. The only exception to this is for the dipole operators, which introduce a new Lorentz structure into EW-top interactions. These operators show consistent, maximal energy growth in the EW sub-amplitudes and are also expected to show some milder growth in the QCD components of processes like $t\bar{t}Z$, $t\bar{t}\gamma$ and $tWj$. Given that these contributions tend to lie roughly two orders of magnitude above the EW versions, energy growing effects in the EW process will take some time to overcome the basic sensitivity offered by the overall rate of the QCD component. That said, identifying these effects provides a clear pathway for the future, when said measurements become systematics dominated and the large statistics can be exploited to measure differential distributions. 

Overall the evidence of energy growth in the sub amplitudes is plain to see, particularly when considering the quadratic EFT contributions, in which the growth compared to the SM is accentuated. However, it is not always possible to see the expected growth in interference contributions.

\begin{figure}[h!]
  \centering 
  \includegraphics[width=\linewidth]{"Images/moneyplot_a3phidql_comb"}
  \caption{ 
  Summary of relative impact on collider processes for $\Opp{\phi Q}{(3)}$ assuming a Wilson coefficient of 1 TeV$^{-2}$. The upper row shows the linear interference contribution while the lower row shows the quadratic piece. The multiple data points per process denote, from left to right starting with the inclusive rate, the impact as a function of cuts designed to access increasingly higher energies. Filled and unfilled bars denote constructive and destructive interference terms respectively, according to the sign conventions in Table~\ref{tab:operators}.
  \label{fig:summary_plot_a3phidql}}
\end{figure}

\begin{figure}[h!]
  \centering 
  \includegraphics[width=\linewidth]{"Images/moneyplot_aphidql_comb"}
  \caption{ 
  Same as Fig.~\ref{fig:summary_plot_a3phidql} for $\Opp{\phi Q}{(1)}$
  \label{fig:summary_plot_aphidql}}
\end{figure}

\begin{figure}[h!]
  \centering 
  \includegraphics[width=\linewidth]{"Images/moneyplot_aphidtr_comb"}
  \caption{ 
  Same as Fig.~\ref{fig:summary_plot_a3phidql} for $\Op{\phi t}$
  \label{fig:summary_plot_aphidtr}}
\end{figure}

\begin{figure}[h!]
  \centering 
  \includegraphics[width=\linewidth]{"Images/moneyplot_atphi_comb"}
  \caption{ 
  Same as Fig.~\ref{fig:summary_plot_a3phidql} for $\Op{t\phi}$
  \label{fig:summary_plot_atphi}}
\end{figure}

\begin{figure}[h!]
  \centering 
  \includegraphics[width=\linewidth]{"Images/moneyplot_atw_comb"}
  \caption{ 
  Same as Fig.~\ref{fig:summary_plot_a3phidql} for $\Op{tW}$
  \label{fig:summary_plot_atw}}
\end{figure}

\begin{figure}[h!]
  \centering 
  \includegraphics[width=\linewidth]{"Images/moneyplot_atb_comb"}
  \caption{ 
  Same as Fig.~\ref{fig:summary_plot_a3phidql} for $\Op{tB}$
  \label{fig:summary_plot_atb}}
\end{figure}
    


==> summary_table.tex <==
{\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\begin{center}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
 \hline
                          & $\Op{\phi D}$ & $\Op{\phi \Box}$ &  $\Op{\phi B}$ & $\Op{\phi W}$  & $\Op{\phi WB}$  & $\Op{W}$ & $\Op{t \phi}$ & $\Op{tB}$ & $\Op{tW}$ & $\Op{\phi Q}^{\sss (1)}$ & $\Op{\phi Q}^{\sss (3)}$ &  $\Op{\phi t}$ & $\Op{\phi tb}$ 
 \tabularnewline\hline
 
 $b\,W\to t\,Z$           & $E$           & $-$              & $-$            & $-$            & $E$             & $E^2$    & $-$           & $E^2$     & $E^2$     & $E$                      & \red{$E^2$}              & $E$            & $E^2$           
 \tabularnewline\hline

 $b\,W\to t\,\gamma$      & $-$           & $-$              & $-$            & $-$            & $E$             & $E^2$    & $-$           & $E^2$     & $E^2$     & $-$                      & $-$                      & $-$            & $-$           
 \tabularnewline\hline
 
 $b\,W\to t\,h$           & $-$           & $-$              & $-$            & $E$            & $-$             & $-$      & $E$           & $-$       & $E^2$     & $-$                      & \red{$E^2$}              & $-$            & $E^2$            
 \tabularnewline\hline
 
 $t\,W\to t\,W$           & $E$           & $E$              & $-$            & $E$            & $E$             & $E^2$    & $E$           & $E$       & $E^2$     & \red{$E^2$}              & \red{$E^2$}              & \red{$E^2$}    & $-$           
 \tabularnewline\hline
 
 $t\,Z\to t\,Z$           & $E$           & $E$              & $E$            & $E$            & $E$             & $-$      & $E$           & $E^2$     & $E^2$     & $E$                      & $E$                      & $E$            & $-$           
 \tabularnewline\hline
 
 $t\,Z\to t\,\gamma$      & $-$           & $-$              & $E$            & $E$            & $E$             & $-$      & $-$           & $E^2$     & $E^2$     & $-$                      & $E$                      & $-$            & $-$           
 \tabularnewline\hline
 
 $t\,\gamma\to t\,\gamma$ & $-$           & $-$              & $E$            & $E$            & $E$             & $-$      & $-$           & $E$       & $E$       & $-$                      & $-$                      & $-$            & $-$           
 \tabularnewline\hline
 
 $t\,Z\to t\,h$           & $E$           & $-$              & $E$            & $E$            & $E$             & $-$      & $E$           & $E^2$     & $E^2$     & \red{$E^2$}              & \red{$E^2$}              & \red{$E^2$}    & $-$           
 \tabularnewline\hline
  
 $t\,\gamma\to t\,h$      & $-$           & $-$              & $E$            & $E$            & $E$             & $-$      & $-$           & $E^2$     & $E^2$     & $-$                      & $-$                      & $-$            & $-$
 \tabularnewline\hline

$t\,h\to t\,h$            & $E$           & $E$              & $-$            & $-$            & $-$             & $-$      & $E$           & $-$       & $-$       & $-$                      & $-$                      & $-$            & $-$           
 \tabularnewline\hline
 
  \end{tabular}
\end{center}
\renewcommand{\arraystretch}{1.}
}


